Answering Ambiguous Questions via Iterative Prompting

In open-domain question answering, due to the ambiguity of questions, multiple plausible answers may exist. To provide feasible answers to an ambiguous question, one approach is to directly predict all valid answers, but this can struggle with balancing relevance and diversity. An alternative is to gather candidate answers and aggregate them, but this method can be computationally costly and may neglect dependencies among answers. In this paper, we present AmbigPrompt to address the imperfections of existing approaches to answering ambiguous questions. Specifically, we integrate an answering model with a prompting model in an iterative manner. The prompting model adaptively tracks the reading process and progressively triggers the answering model to compose distinct and relevant answers. Additionally, we develop a task-specific post-pretraining approach for both the answering model and the prompting model, which greatly improves the performance of our framework. Empirical studies on two commonly-used open benchmarks show that AmbigPrompt achieves state-of-the-art or competitive results while using less memory and having a lower inference latency than competing approaches. Additionally, AmbigPrompt also performs well in low-resource settings. The code are available at: https://github.com/sunnweiwei/AmbigPrompt.

==> tables/ambigqa.tex <==
\begin{table*}[!t]
\centering
\setlength\tabcolsep{7pt}
\begin{tabular}{@{}llll cccc@{}}

\toprule

\multirow{2}{*}{\textbf{Methods}}
&  \multirow{2}{*}{\textbf{\#Params}} & \multirow{2}{*}{\textbf{Latency}} &\multirow{2}{*}{\textbf{Memory}}
& \multicolumn{2}{c}{\textbf{Dev}}
& \multicolumn{2}{c}{\textbf{Test}}
\\

\cmidrule(lr){5-6} \cmidrule(lr){7-8} 

&&& & Full & Multi & Full & Multi
\\
\midrule

DPR~\citep{Karpukhin2020DensePR} & 345M\quad $1.0\times$ & ~~0.37s\quad $1.0\times$ & ~~4GB\quad $1.0\times$ & 43.5 & 34.6 & 39.6 & 31.4 \\

SpanSeqGen~\citep{Min2020AmbigQAAA} & 400M\quad $1.2\times$ & ~~0.49s\quad $1.3\times$ & ~~5GB\quad $1.3\times$ & 42.3 & 31.7 & 35.9 & 26.0 \\

FiD~\citep{Izacard2021LeveragingPR} & 220M\quad $0.6\times$ & ~~0.38s\quad $1.0\times$ & ~~4GB\quad $1.0\times$ & 45.5 & 35.8 & 39.6 & 31.4 \\

Refuel$^\dagger$~\citep{Gao2021AnsweringAQ} & 400M\quad $1.2\times$ & 22.19s\quad $58.6\times$  & ~~8GB\quad $2.0\times$ & 48.3 & 37.3 & 42.1 & 33.3 \\

JPR$^\dagger$~\citep{Min2021JointPR} & 3B\quad\quad~$8.7\times$ & ~~0.88s\quad $2.3\times$  & 14GB\quad $3.5\times$ & 48.5 & 37.6 & 43.5 & 34.2 \\

RECTIFY$^\dagger$~\citep{Shao2021AnsweringOM} & 6B\quad\quad~$17.4\times$ & 19.72s\quad $51.3\times$ & 14GB\quad $3.5\times$ & 52.1 & 41.6 & 46.2 & 37.1 \\

\midrule
\textbf{AmbigPrompt} & 220M\quad $0.6\times$ & ~~0.68s\quad $1.8\times$ & ~~4GB\quad $1.0\times$ & 48.7 & 38.8 & 43.9 & 36.6  \\

\bottomrule
\end{tabular}
\caption{Question Answering results on AmbigQA~\citep{Min2020AmbigQAAA}. Full and Multi denote the full set and multi-answer set respectively. The reported value is F1. Methods with $^\dagger$ have no publicly available codes, therefore we estimate the values of latency and memory with randomly initialized models.} \label{table:ambigqa}
\end{table*}


==> tables/hyper-param.tex <==
\begin{table}[h]
\centering \small
\setlength\tabcolsep{12pt}
\begin{tabular}{l cc c}

\toprule

Method & Full  & Multi \\
\midrule
AmbigPrompt & 48.7 & 38.8\\
\midrule
\multicolumn{3}{@{}l}{\emph{Number of passages}}\\
- $m=50$ & 43.8 & 35.1\\
- $m=10$ & 39.1 & 32.4\\

\midrule
\multicolumn{3}{@{}l}{\emph{Decoding method}}\\
- Beam=3 & 47.2 & 37.6 \\

\bottomrule
\end{tabular}
\caption{Hyper-parameter analysis on AmbigQA dev.}
\label{table:hyper}
\end{table}


==> tables/main2.tex <==
\begin{table*}[!t]
\centering \small
\setlength\tabcolsep{6pt}
\begin{tabular}{@{}l rr rr rr rrrr@{}}

\toprule

\multirow{2}{*}{\textbf{Methods}}
&  \multicolumn{2}{r}{\multirow{2}{*}{\textbf{\#Params}}} 
& \multicolumn{2}{r}{\multirow{2}{*}{\textbf{Latency}}}
&\multicolumn{2}{r}{\multirow{2}{*}{\textbf{Memory}}}
& \multicolumn{2}{r}{\textbf{AmbigQA}}
& \multicolumn{2}{r}{\textbf{WebQSP}}
\\

\cmidrule(lr){8-9} \cmidrule(lr){10-11} 

&&&&&& & Full & Multi & Full & Multi
\\
\midrule

DPR~\citep{Karpukhin2020DensePR} & 345M & $1.0\times$ & 0.37s & $1.0\times$ & 4GB & $1.0\times$ & 43.5 & 34.6 & 51.9 & 45.0 \\

SpanSeqGen~\citep{Min2020AmbigQAAA} & 400M & $1.2\times$ & ~~0.49s & $1.3\times$ & 5GB & $1.3\times$ & 42.3 & 31.7 & - & - \\

FiD-Base~\citep{Izacard2021LeveragingPR} & 220M & $0.6\times$ & 0.38s & $1.0\times$ & 4GB & $1.0\times$ & 45.5 & 35.8 & 51.9 & 45.0 \\

Refuel$^\dagger$~\citep{Gao2021AnsweringAQ} & 400M & $1.2\times$ & 22.19s & $58.6\times$  & 8GB & $2.0\times$ & 48.3 & 37.3 & - & - \\

\midrule
\emph{High capacity models}\\
JPR$^\dagger$~\citep{Min2021JointPR} & 3B & $8.7\times$ & 0.88s & $2.3\times$  & 14GB & $3.5\times$ & 48.5 & 37.6 & 53.1 & 47.2 \\

RECTIFY$^\dagger$~\citep{Shao2021AnsweringOM} & 6B & $17.4\times$ & 19.72s & $51.3\times$ & 14GB & $3.5\times$ & 52.1 & 41.6 & 55.8 & 48.8 \\

\midrule
\textbf{AmbigPrompt} & 220M & $0.6\times$ & 0.68s & $1.8\times$ & 4GB & $1.0\times$ & 48.7 & 38.8 & 53.2 & 47.9  \\
\midrule
\emph{Ablative variants}\\
- w/o pre-training & & & & & & & 40.8 & 31.4 & 47.4 & 39.2 \\
- w/o prompting model & & & & & & & 46.0 & 34.3 & 49.7 & 44.6 \\
- w/o interleaving prompting & & & & & & & 47.8 & 36.9 & 50.9 & 45.4 \\

\bottomrule
\end{tabular}
\caption{Compare with state-of-the art methods in AmbigQA~\citep{Min2020AmbigQAAA} and WebQSP~\citep{Yih2016TheVO} in terms of efficiency and effectiveness. Full and Multi denote the full set and multi-answer set respectively. The reported value is F1. Methods with $^\dagger$ have no publicly available codes, therefore we estimate the values of latency and memory with randomly initialized models.} \label{table:ambigqa}
\end{table*}


==> tables/prompt.tex <==
\begin{table}[!t]
\centering \small
\setlength\tabcolsep{4pt}
\caption{Zero-shot evaluation results on AmbigQA~\citep{Min2020AmbigQAAA}, The reported value is F1. In zero-shot setting, the models do not use AmbigQA training set.}
\label{prompt}

\begin{tabular}{@{}l cc cc@{}}

\toprule

{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{Zero-shot}}
& \multicolumn{2}{c}{\textbf{Supervised}}
\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} 

& Full & Multi & Full & Multi\\
\midrule
Concatenation & 41.2 & 30.4 & 45.4 & 34.8 \\
Beam search & 40.6 & 33.5 & - & - \\
Prompt & 46.5 & 37.9 & 48.7 & 38.8 \\

\bottomrule
\end{tabular}
\end{table}


==> tables/qam.tex <==
\begin{table}[!t]
\centering  \small
\setlength\tabcolsep{3pt}
\caption{Question Answering results on QAMParI~\citep{Rubin2022QAMPARIA} and NQ~\citep{Kwiatkowski2019NaturalQA}. Results of baselines are copyed from \citet{Rubin2022QAMPARIA}.}
\begin{tabular}{@{}l cccc c@{}}

\toprule
& Recall & Precision & F1 & \%F1$\ge$0.5 & NQ-EM \\
\midrule
RAG-Base &  49.7 & 22.0 & 24.9 & 13.0 & - \\
RAG-Large & 52.4 & 21.6 & 26.6 & 15.3 & -\\
FiD-Base & 14.2 & 32.6 & 18.2 & 11.0 & 35.2 \\
FiD-Large & 19.0 & 34.5 & 22.7 & 16.9 & 41.2\\
% \midrule\textbf{AmbigPrompt} & 53.3 & 46.7 & 53.2 & 47.9 & 49.2 \\


\bottomrule
\end{tabular}
\end{table}


==> tables/webqsp.tex <==
\begin{table}[!t]
\centering \small
\setlength\tabcolsep{3pt}
\caption{Question Answering results on WebQSP~\citep{Yih2016TheVO} and QAMParI~\citep{Rubin2022QAMPARIA}.}
\begin{tabular}{@{}l cccc c@{}}

\toprule

{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{WebQSP-Dev}}
& \multicolumn{2}{c}{\textbf{WebQSP-Test}} & \multicolumn{1}{c}{\textbf{QAMParI}}
\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-6} 

& Full & Multi & Full & Multi & Test\\
\midrule
DPR & 50.7 & 45.3 & 51.9 & 45.0 & -  \\
JPR &  53.6 & 49.5 & 53.1 & 47.2 & - \\
RECTIFY & 55.4 & 45.4 & 55.8 & 48.8 & - \\
RAG-Large & - & - & - & - & 26.6 \\
FiD-Base & - & - & - & - & 19.2 \\
FiD-Large & - & - & - & - & 25.1 \\
\midrule\textbf{AmbigPrompt} & 53.3 & 46.7 & 53.2 & 47.9 & 31.2 \\


\bottomrule
\end{tabular}
\end{table}

